UVA: Towards Unified Volumetric Avatar for View Synthesis, Pose rendering, Geometry and Texture Editing

Neural radiance field (NeRF) has become a popular 3D representation method for human avatar reconstruction due to its high-quality rendering capabilities, e.g., regarding novel views and poses. However, previous methods for editing the geometry and appearance of the avatar only allow for global editing through body shape parameters and 2D texture maps. In this paper, we propose a new approach named \textbf{U}nified \textbf{V}olumetric \textbf{A}vatar (\textbf{UVA}) that enables local and independent editing of both geometry and texture, while retaining the ability to render novel views and poses. UVA transforms each observation point to a canonical space using a skinning motion field and represents geometry and texture in separate neural fields. Each field is composed of a set of structured latent codes that are attached to anchor nodes on a deformable mesh in canonical space and diffused into the entire space via interpolation, allowing for local editing. To address spatial ambiguity in code interpolation, we use a local signed height indicator. We also replace the view-dependent radiance color with a pose-dependent shading factor to better represent surface illumination in different poses. Experiments on multiple human avatars demonstrate that our UVA achieves competitive results in novel view synthesis and novel pose rendering while enabling local and independent editing of geometry and appearance. The source code will be released.

==> fig_tex/abl_visu.tex <==
\begin{figure*}[htbp]
    \centering
    % \setlength\tabcolsep{.5pt} % default value: 6pt
    \includegraphics[width=1\linewidth]{figures/ablation_visu.pdf}
    \caption{\textit{Visual results} of ablation study. }
    \label{fig:ablation}
\end{figure*}

==> tables/NV_NP_zju_aver.tex <==
\begin{table*}
\scriptsize
 \centering
 \setlength{\tabcolsep}{3pt}
 \renewcommand{\arraystretch}{1.1}
 \begin{tabular}{ | c | c | c | c |  c | c | c  | c | c | c | c | c | c |}
 \hline
 & \multicolumn{3}{c|}{313} & \multicolumn{3}{c|}{315} & \multicolumn{3}{c|}{377} & \multicolumn{3}{c|}{387}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline
    Ani-N & 29.8 & 0.963 & 0.075 & 23.1 & 0.917 & 0.138 & 24.2 & 0.925 & 0.124 & 25.4 & 0.926 & 0.131 \\
   % \hline
    A-NeRF & 29.2 & 0.954 & 0.075 & 25.1 & 0.948 & 0.087 & 27.2 & 0.951 & 0.080 & 26.3 & 0.937 & 0.100 \\
    % \hline
    NB & 30.5 & 0.967 & 0.068 & 26.4 & 0.958 & 0.079 & {28.1} & {0.956} & 0.080 & 26.7 & 0.942 & 0.101 \\
    % 
    ARAH & {31.6} & {0.973} & {0.050} & {27.0} & {0.965} & {0.058} & 27.8 & {0.956} & {0.071} & {27.0} & {0.945} & {0.079} \\
    %
    TAVA-NN & 29.6 & 0.961 & 0.062 & 24.6 & 0.930 & 0.102  & 26.5 & 0.938 &  0.094 & 24.9 & 0.909 & 0.130 \\
    % \hline
    Ours & 30.7 & 0.963 & 0.063 & 26.9 & 0.953  & 0.093  & 28.1  & 0.957 & 0.086 & 26.7 & 0.930 & 0.118\\
    %
    
 % \hline
 % & \multicolumn{3}{c|}{386} & \multicolumn{3}{c|}{387} & \multicolumn{3}{c|}{390}
 % \\\hline
 % Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 % \hline
 % Ani-N & 25.6 & 0.878 & 0.199 & 25.4 & 0.926 & 0.131 & 26.0 & 0.912 & 0.148 \\
 % % % \hline
 % A-NeRF & 28.5 & 0.928 & 0.127 & 26.3 & 0.937 & 0.100 & 27.0 & 0.914 & 0.126 \\
 %  % \hline
 % NB & 29.0 & {0.935} & 0.112 & 26.7 & 0.942 & 0.101 & {27.9} & 0.928 & 0.112 \\
 % % 
 %  ARAH & {29.2} & 0.934 & {0.105}  & {27.0} & {0.945} & {0.079} & {27.9} & {0.929} & {0.102} \\
 %  %
 % TAVA-NN & 26.9 & 0.927 & 0.120  & 24.9 & 0.909 & 0.130  & 26.5 & 0.911 & 0.122 \\
 % % \hline
 % Ours & 30.7  & 0.951 & 0.104  & 26.7 & 0.930 & 0.118 & 26.4 & 0.918 & 0.142  \\
 % % \hline

 % \hline
 % & \multicolumn{3}{c|}{392} & \multicolumn{3}{c|}{393} & \multicolumn{3}{c|}{394}
 % \\\hline
 %  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 % \hline


 % Ani-N & 28.0 & 0.931 & 0.151 & 26.1 & 0.916 & 0.151 & 27.5 & 0.924 & 0.142 \\
 % % % \hline
 % A-NeRF & 28.7 & 0.942 & 0.106 & 26.8 & 0.931 & 0.113 & 28.1 & 0.936 & 0.103 \\
 %  % \hline
 %  NB & {29.7} & {0.949} & 0.101 & {27.7} & 0.939 & 0.105 & 28.7 & 0.942 & 0.098 \\
 %  %
 %   ARAH & 29.5 & 0.948 & {0.090} & {27.7} & {0.940} & {0.093} & {28.9} & {0.945} & {0.084} \\
 %   %
 %    TAVA-NN & 26.8 & 0.924 & 0.119  & 25.2 & 0.908 & 0.131  & 26.1 & 0.911 & 0.131  \\
 %    % \hline
 %    Ours & 28.1  & 0.937  & 0.126  & 26.1  & 0.920  & 0.139 & 28.1  & 0.934  & 0.119  \\
 % % \hline

 \hline
 \end{tabular}

  \caption{\textbf{Novel View Synthesis.} We report PSNR, SSIM, and LPIPS~\cite{zhang2018perceptual} for novel views of training poses of the ZJU-MoCap dataset~\cite{peng2020neural}. Due to better geometry, our approach produces more consistent rendering results across novel views than the baselines. We include qualitative comparisons in \iftoggle{arXiv}{Appendix~\ref{appx:additional_qualitative_train}.}{the Supp. Mat.} Note that we crop slightly larger bounding boxes than Neural Body~\cite{peng2020neural} to better capture loose clothes, \eg\ sequence 387 and 390. Therefore, the reported numbers vary slightly from their evaluation.}
 % \iftoggle{arXiv}{\vspace{0.05in}}{}
 \label{tab:novel_view}
 
\end{table*}

==> tables/comparison_zju.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}
\vspace*{-1.5em}
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l cc cc cc}
%\hline\hline\noalign{\smallskip}
\toprule
& \multicolumn{2}{c}{Novel-view} & \multicolumn{2}{c}{Novel-pose (ind)} & \multicolumn{2}{c}{Novel-pose (ood)} \\
& PSNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\
\midrule%\hline
\noalign{\smallskip}
\emph{\underline{\textbf{SMPL-based Methods}}} & & & & & & \\
Animatable-NeRF~\cite{peng2021animatable} & 30.75 & 0.971 & 29.34 & 0.966 & 28.67 & 0.961 \\
NeuralBody~\cite{peng2021neural} & \textbf{33.91} & \textbf{0.983} & \textbf{33.43} & \textbf{0.984} & \textbf{30.33} & \textbf{0.969} \\
\emph{\underline{\textbf{Template-free Methods}}} & & & & & & \\
Pose-NeRF & 31.88 & 0.975 & 32.09 & 0.976 & 28.43 & 0.954 \\
A-NeRF~\cite{su2021nerf} & 32.45 & 0.978 & 32.65 & 0.978 & 30.41 & 0.967 \\
NARF~\cite{noguchi2021neural} & 32.94 & 0.980 & 33.21 & 0.980 & 30.60 & 0.968 \\
\hline\noalign{\smallskip}
Tava & \textbf{33.11} & \textbf{0.981} & \textbf{33.35} & \textbf{0.981} & \textbf{30.69} & \textbf{0.969} \\
Ours & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\bottomrule
%\hline\hline
\end{tabular}
}
\end{center}
\vspace*{-0.8em}
\caption{\textit{Comparisons on the ZJU Mocap subjects}. We compare with both, template-free and template-based  methods.}
\vspace*{-5em}
\label{tab:comparison_zju}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

==> tables/novel_pose_zju.tex <==
\begin{table*}
\scriptsize
 \renewcommand{\tabcolsep}{3.0pt}

 \centering
 \begin{tabular}{ | c | c | c | c |  c | c | c  | c | c | c | }
 \hline
 & \multicolumn{3}{c|}{313} & \multicolumn{3}{c|}{315} & \multicolumn{3}{c|}{377}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline
 Ani-N & 23.9 & 0.909 & 0.115 & 19.2 & 0.855 & 0.167 & 22.6 & 0.900 & 0.153 \\
 % % \hline
 A-NeRF & 22.0 & 0.855 & 0.209 & 18.7 & 0.810 & 0.232 & 22.6 & 0.890 & 0.165 \\
 % \hline
  NB & 24.1 & 0.908 & 0.126 & 19.8 & 0.867 & 0.152 & 24.2 & 0.917 & 0.119 \\
  % 
   ARAH & {24.4} & {0.914} & {0.092} & {20.0} & {0.881} & {0.105} & {25.5} & {0.933} & {0.093} \\
   %
  TAVA-NN & 23.52 & 0.917 & 0.096  & 19.7 & 0.884 & 0.122 & 24.2 & 0.901 & 0.131  \\
  % 
  Ours & 24.7   & 0.904  & 0.119  & 20.2  & 0.893  & 0.119  &  25.5 & 0.922  & 0.126  \\
  %

 
 \hline
 & \multicolumn{3}{c|}{386} & \multicolumn{3}{c|}{387} & \multicolumn{3}{c|}{390}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline

 Ani-N & 25.5 & 0.884 & 0.187 & 23.1 & 0.906 & 0.145 & 23.9 & 0.887 & 0.173 \\
 % % \hline
 A-NeRF & 24.8 & 0.858 & 0.241 & 22.4 & 0.885 & 0.162 & 22.6 & 0.846 & 0.226 \\
 %
  NB & 26.1 & 0.894 & 0.171 & 22.7 & 0.902 & 0.135 & 24.2 & 0.882 & 0.164 \\
   %
   ARAH & {27.0} & {0.910} & {0.127} & {24.2} & {0.917} & {0.099} & {24.8} & {0.896} & {0.126} \\
 % \hline
 TAVA-NN & 24.5 & 0.875 & 0.178  & 23.1 & 0.883 & 0.152  & 24.4 & 0.879 & 0.156  \\
 % 
 Ours & 26.7  & 0.901  & 0.165  & 24.0  & 0.898  & 0.140  & 25.58  & 0.898  & 0.168  \\
 %

 
 \hline
 & \multicolumn{3}{c|}{392} & \multicolumn{3}{c|}{393} & \multicolumn{3}{c|}{394}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline
 
 % \hline
 Ani-N & 24.3 & 0.900 & 0.169 & 23.8 & 0.897 & 0.155 & 24.1 & 0.887 & 0.171 \\
 % % \hline
 A-NeRF & 23.7 & 0.886 & 0.183 & 22.1 & 0.875 & 0.175 & 22.7 & 0.861 & 0.199 \\
 % 
 NB & 26.0 & 0.916 & 0.135 & 23.5 & 0.900 & 0.132 & 24.1 & 0.888 & 0.150 \\
 % 
  ARAH & {26.2} & {0.927} & {0.106} & {24.4} & {0.915} & {0.104} & {25.2} & {0.908} & {0.111} \\
  %
 TAVA-NN & 25.3 & 0.904 & 0.139  & 24.1 & 0.897 & 0.136  & 24.6 & 0.892 & 0.143 \\
 %
 Ours & 25.4  & 0.907  & 0.151  & 25.2  & 0.918  & 0.118  &  24.7 & 0.915  & 0.128  \\
 % \hline

 \hline
 \end{tabular}

  \caption{\textbf{Novel Pose Rendering.}  PSNR, SSIM, LPIPS \cite{zhang_UnreasonableEffectivenessDeep_2018} are reported for the test poses of the ZJU-MoCap dataset \cite{pengNeuralBodyImplicit2021}.}
 % \iftoggle{arXiv}{\vspace{0.05in}}{}
 \label{tab:novel_pose}
 
\end{table*}

==> tables/novel_view_zju.tex <==
\begin{table*}
\scriptsize
 \centering
 \setlength{\tabcolsep}{3pt}
 \renewcommand{\arraystretch}{1.1}
 \begin{tabular}{ | c | c | c | c |  c | c | c  | c | c | c | }
 \hline
 & \multicolumn{3}{c|}{313} & \multicolumn{3}{c|}{315} & \multicolumn{3}{c|}{377}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline
    Ani-N & 29.8 & 0.963 & 0.075 & 23.1 & 0.917 & 0.138 & 24.2 & 0.925 & 0.124 \\
   % \hline
    A-NeRF & 29.2 & 0.954 & 0.075 & 25.1 & 0.948 & 0.087 & 27.2 & 0.951 & 0.080 \\
    % \hline
    NB & 30.5 & 0.967 & 0.068 & 26.4 & 0.958 & 0.079 & {28.1} & {0.956} & 0.080 \\
    % 
    ARAH & {31.6} & {0.973} & {0.050} & {27.0} & {0.965} & {0.058} & 27.8 & {0.956} & {0.071} \\
    %
    TAVA-NN & 29.6 & 0.961 & 0.062 & 24.6 & 0.930 & 0.102  & 26.5 & 0.938 &  0.094 \\
    % \hline
    Ours & 30.7 & 0.963 & 0.063 & 26.9 & 0.953  & 0.093  & 28.1  & 0.957 & 0.086 \\
    %
    
 \hline
 & \multicolumn{3}{c|}{386} & \multicolumn{3}{c|}{387} & \multicolumn{3}{c|}{390}
 \\\hline
 Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline
 Ani-N & 25.6 & 0.878 & 0.199 & 25.4 & 0.926 & 0.131 & 26.0 & 0.912 & 0.148 \\
 % % \hline
 A-NeRF & 28.5 & 0.928 & 0.127 & 26.3 & 0.937 & 0.100 & 27.0 & 0.914 & 0.126 \\
  % \hline
 NB & 29.0 & {0.935} & 0.112 & 26.7 & 0.942 & 0.101 & {27.9} & 0.928 & 0.112 \\
 % 
  ARAH & {29.2} & 0.934 & {0.105}  & {27.0} & {0.945} & {0.079} & {27.9} & {0.929} & {0.102} \\
  %
 TAVA-NN & 26.9 & 0.927 & 0.120  & 24.9 & 0.909 & 0.130  & 26.5 & 0.911 & 0.122 \\
 % \hline
 Ours & 30.7  & 0.951 & 0.104  & 26.7 & 0.930 & 0.118 & 26.4 & 0.918 & 0.142  \\
 % \hline

 \hline
 & \multicolumn{3}{c|}{392} & \multicolumn{3}{c|}{393} & \multicolumn{3}{c|}{394}
 \\\hline
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
 \hline


 Ani-N & 28.0 & 0.931 & 0.151 & 26.1 & 0.916 & 0.151 & 27.5 & 0.924 & 0.142 \\
 % % \hline
 A-NeRF & 28.7 & 0.942 & 0.106 & 26.8 & 0.931 & 0.113 & 28.1 & 0.936 & 0.103 \\
  % \hline
  NB & {29.7} & {0.949} & 0.101 & {27.7} & 0.939 & 0.105 & 28.7 & 0.942 & 0.098 \\
  %
   ARAH & 29.5 & 0.948 & {0.090} & {27.7} & {0.940} & {0.093} & {28.9} & {0.945} & {0.084} \\
   %
    TAVA-NN & 26.8 & 0.924 & 0.119  & 25.2 & 0.908 & 0.131  & 26.1 & 0.911 & 0.131  \\
    % \hline
    Ours & 28.1  & 0.937  & 0.126  & 26.1  & 0.920  & 0.139 & 28.1  & 0.934  & 0.119  \\
 % \hline

 \hline
 \end{tabular}

  \caption{\textbf{Novel View Synthesis.} We report PSNR, SSIM, and LPIPS~\cite{zhang_UnreasonableEffectivenessDeep_2018} of novel view synthesis for the nine performers of the ZJU-MoCap dataset~\cite{pengNeuralBodyImplicit2021}.}
 % \iftoggle{arXiv}{\vspace{0.05in}}{}
 \label{tab:novel_view}
 
\end{table*}
